Dynamic Importance in Diffusion U-Net for Enhanced Image Synthesis

Traditional diffusion models typically employ a U-Net architecture. Previous studies have unveiled the roles of attention blocks in the U-Net. However, they overlook the dynamic evolution of their importance during the inference process, which hinders their further exploitation to improve image applications. In this study, we first theoretically proved that, re-weighting the outputs of the Transformer blocks within the U-Net is a "free lunch" for improving the signal-to-noise ratio during the sampling process. Next, we proposed Importance Probe to uncover and quantify the dynamic shifts in importance of the Transformer blocks throughout the denoising process. Finally, we design an adaptive importance-based re-weighting schedule tailored to specific image generation and editing tasks. Experimental results demonstrate that, our approach significantly improves the efficiency of the inference process, and enhances the aesthetic quality of the samples with identity consistency. Our method can be seamlessly integrated into any U-Net-based architecture. Code: https://github.com/Hytidel/UNetReweighting

==> algorithm-figure-table/alg/alg-weight_threshold_update.tex <==
% ---------= 伪代码中出现的操作 =---------
% 多参数 Input 的首个参数
\newcommand{\MultiInput}[1]{
  \textbf{Input:} 
  \begin{itemize}[leftmargin = 2em, noitemsep, topsep = 0pt]
    \item #1
  \end{itemize}
}

% 多参数 Output 的首个参数
\newcommand{\MultiOutput}[1]{
  \textbf{Output:} 
  \begin{itemize}[leftmargin = 2em, noitemsep, topsep = 0pt]
    \item #1
  \end{itemize}
}

% 增加参数
\newcommand{\AddItem}[1]{
  \begin{itemize}[leftmargin = 2em, noitemsep, topsep = 0pt]
    \item #1
  \end{itemize}
}

% 阈值更新过程伪代码
\begin{algorithm}
\caption{Importance Probe in a Epoch}
    % Input
    \MultiInput{\text{weight\_threshold\_matrix}}
    \AddItem{\text{history\_best\_weight\_matrix}}
    \AddItem{\text{letents}, \text{conditions}}


    \vspace{5pt}
    
    \begin{algorithmic}[1]
        \State $\text{weight\_threshold\_list} \newline
        \hspace*{10pt} \leftarrow \text{weight\_threshold\_matrix}[\text{inference\_step}]$
        \State $\text{best\_fitness} \leftarrow \text{cal\_fitness}(\text{weight\_threshold\_list})$
        \State
        \State $\text{best\_weight\_list} \leftarrow \varnothing$
        \State $\text{accepted\_mask} \leftarrow [\text{False}] \times \text{num\_inference\_step}$

        \State
        
        \For{$\text{inference\_step} = 0$ to $(\text{num\_inference\_step} - 1)$}
            \State $\text{time\_step} \leftarrow \text{time\_steps}[\text{inference\_step}]$
            \State $\epsilon_{\text{tea}} \leftarrow \text{tea\_U-Net}(\text{letents}, \text{conditions}, \text{time\_step})$
            
            \State 
            
            \State $\text{cur\_weight\_list} \newline 
            \hspace*{20pt} \leftarrow \text{history\_best\_weight\_matrix}[\text{inference\_step}]$
            
            \For{$\text{stu\_try} = 1$ to $(\text{num\_stu\_try} - 1)$}
                \State $\text{weight\_list}$ \newline 
                    \hspace*{40pt} $\leftarrow \text{WeightBiasSchedule}(\text{cur\_weight\_list})$ 
                
                \State $\text{stu\_U-Net.set\_weight}(\text{weight\_list})$
                
                \State $\epsilon_{\text{stu}} \leftarrow \text{stu\_U-Net}(\text{letents},  \text{conditions}, \text{time\_step})$

                \State 
                
                \If{$\text{criterion}(\epsilon_{\text{tea}}, \epsilon_{\text{stu}}) \leq \text{loss\_threshold}$}
                    \State $\text{tmp\_fitness} = \text{cal\_fitness}(\text{weight\_list})$
                    \If{$\text{tmp\_fitness} > \text{best\_fitness}$}
                        \State $\text{best\_fitness} \leftarrow \text{tmp\_fitness}$
                        \State $\text{best\_weight\_list} \leftarrow \text{weight\_list}$
                    \EndIf
                \EndIf
            \EndFor
            \State
            \If{$\text{best\_weight\_list} == \varnothing$}
                \State $\text{weight\_threshold\_matrix}[\text{inference\_step}]$ \newline
                    \hspace*{40pt} $\leftarrow \text{cur\_weight\_list}$
            \Else
                \State $\text{accepted\_mask}[\text{inference\_step}] \leftarrow \text{True}$
                \State $\text{weight\_threshold\_matrix}[\text{inference\_step}]$ \newline
                    \hspace*{40pt} $\leftarrow \text{best\_weight\_list}$
                \State $\text{history\_best\_weight\_matrix}[\text{inference\_step}]$ \newline
                    \hspace*{40pt} $\leftarrow \text{best\_weight\_list}$
            \EndIf

            \State 

            \State $\text{latents} \leftarrow \text{scheduler.step}(\text{latents}, \epsilon_{\text{tea}}, \text{time\_step})$
        \EndFor

        \State 

        \State $\text{weight\_threshold\_matrix}$ \newline
            \hspace*{10pt} $\leftarrow \text{ThresholdUpdateScheduler}(\text{accepted\_mask})$
    \end{algorithmic}
\label{alg-weight_threshold_update}
\end{algorithm}

==> algorithm-figure-table/fig/fig-bar_chart_voting_score-sd.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{c c c c c}
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/0.png} 
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/1.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/2.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/3.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/4.png}

        \\ 

        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/5.png} 
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/6.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/7.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/8.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/9.png}
        
        \\

        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/10.png} 
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/11.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/12.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/13.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/14.png}

        \\ 

        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/15.png} 
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/16.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/17.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/18.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd/19.png}
    \end{tabular}
    \captionof{figure}{
        Bar charts of voting scores for SD v2.1. 
    }
    \label{tab-bar_chart_voting_score-sd}
\end{table*}


==> algorithm-figure-table/fig/fig-bar_chart_voting_score-sdturbo-dog.tex <==
\begin{figure}[ht]
    \centering
    % 图: voting score in step-0
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=0.98\linewidth]{algorithm-figure-table/bar_chart_voting_score/bar_chart_0.png}
        \caption{inference step - 0}
    \end{subfigure}
    \hfill
    % 图: voting score in step-1
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=0.98\linewidth]{algorithm-figure-table/bar_chart_voting_score/bar_chart_1.png}
        \caption{inference step - 1}
    \end{subfigure}
    \caption{Bar charts of voting scores for all blocks at every inference step. }
    \label{fig-bar_chart_voting_score-sdturbo-dog}
\end{figure}



==> algorithm-figure-table/fig/fig-bar_chart_voting_score-sdturbo.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=0.45\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd-turbo/0.png} 
        & 
        \includegraphics[width=0.45\linewidth]{algorithm-figure-table/bar_chart_voting_score/sd-turbo/1.png}
    \end{tabular}
    \captionof{figure}{
        Bar charts of voting scores for SD-Turbo. 
    }
    \label{tab-bar_chart_voting_score-sdturbo}
\end{table}


==> algorithm-figure-table/fig/fig-bar_chart_voting_score-sdxl.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{c c c c c}
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/0.png} 
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/1.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/2.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/3.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/4.png}

        \\ 

        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/5.png} 
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/6.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/7.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/8.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/9.png}
        
        \\

        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/10.png} 
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/11.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/12.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/13.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/14.png}

        \\ 

        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/15.png} 
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/16.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/17.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/18.png}
        & 
        \includegraphics[width=0.175\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl/19.png}
    \end{tabular}
    \captionof{figure}{
        Bar charts of voting scores for SDXL. 
    }
    \label{tab-bar_chart_voting_score-sdxl}
\end{table*}


==> algorithm-figure-table/fig/fig-bar_chart_voting_score-sdxlturbo.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=0.45\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl-turbo/0.png} 
        & 
        \includegraphics[width=0.45\linewidth]{algorithm-figure-table/bar_chart_voting_score/sdxl-turbo/1.png}
    \end{tabular}
    \captionof{figure}{
        Bar charts of voting scores for SDXL-Turbo. 
    }
    \label{tab-bar_chart_voting_score-sdxlturbo}
\end{table}


==> algorithm-figure-table/fig/fig-dynamic_pruning.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\linewidth]{algorithm-figure-table/fig/dynamic_pruning.png}
    \caption{
        The schematic of dynamic pruning of SD U-Net, in which the gray rectangles represent the skipped Transformer blocks in that step. 
    }
    \label{fig-dynamic_pruning}
    \vspace{-10pt}
\end{figure}

==> algorithm-figure-table/fig/fig-failure_case.tex <==
% importance-based re-weighting, SDXL-Turbo, 2
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c c}
        \hline

        \multirow{2}{*}{\textbf{Models}} & \multicolumn{4}{c}{\textbf{Re-weighting Schedule}} \\
        ~ & Vanilla & $[0.98, 1.1]$ / $[0.95, 1.1]$ & $[0.98, 1.15]$ / $[0.95, 1.15]$ & $[0.98, 1.2]$ / $[0.95, 1.2]$ \\
        
        \hline

        \rule{0pt}{0pt} \\
        
        % SD-Turbo
        \parbox[t][-2.75cm][c]{2.0cm}{\centering SD-Turbo} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/failure_base/sd-turbo/default.png} & \includegraphics[width=0.15\textwidth]{algorithm-figure-table/failure_base/sd-turbo/0.98_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/failure_base/sd-turbo/0.98_1.15.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/failure_base/sd-turbo/0.98_1.2.png} \\

        % SDXL-Turbo
        \parbox[t][-2.75cm][c]{2.0cm}{\centering SDXL-Turbo} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/failure_base/sdxl-turbo/default.png} & \includegraphics[width=0.15\textwidth]{algorithm-figure-table/failure_base/sdxl-turbo/0.95_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/failure_base/sdxl-turbo/0.95_1.15.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/failure_base/sdxl-turbo/0.95_1.2.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \captionof{figure}{
        Failure cases of SD-Turbo and SDXL-Turbo under the optimal re-weighting schedules. 
    }
    \label{fig-failure_case}
\end{table*}



==> algorithm-figure-table/fig/fig-fid_lpips_fruit_all.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\linewidth]{algorithm-figure-table/scatter-dog_metric/scatter_metric_sdturbo_dog.png}
    \caption{
        Scatter plot of FID and LPIPS under different skipping strategies. 
        (the further lower-left, the better).
        Baseline strategies are represented by blue circles, unique points from our strategies are shown as pink circles, while points overlapping with baseline points are marked with purple stars. 
    }
    \label{fig-fid_lpips_fruit_all}
    \vspace{-10pt}
\end{figure}


==> algorithm-figure-table/fig/fig-freeu_failure.tex <==
% 表: FreeU 失败的情况
\begin{table}[h]
    \centering
    % 3 images
    \begin{tabular}{c | c c}
    
        \hline
        
        \textbf{Standard SD-Turbo} & \textbf{+ FreeU} & \textbf{Our Enhanced} \\
        
        \hline

        \rule{0pt}{0pt} \\
    
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/freeu_failure/default.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/freeu_failure/0.9_1.4_0.2_1.6_noted.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/freeu_failure/1.0_1.1_noted.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}

    \captionof{figure}{
        FreeU fails to preserve the identity consistency, whereas Ours enhances the visual quality while preserving the identity. 
    }
    \label{fig-freeu_failure}
\end{table}


==> algorithm-figure-table/fig/fig-heatmap_importance_score-sd.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{algorithm-figure-table/heatmap_importance_score/sd.png}
    \caption{
        Heatmap of importance scores for SD v2.1. 
    }
    \label{fig-heatmap_importance_score-sd}
\end{figure}


==> algorithm-figure-table/fig/fig-heatmap_importance_score-sdturbo.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{algorithm-figure-table/heatmap_importance_score/sd-turbo.png}
    \caption{
        Heatmap of importance scores for SD-Turbo.  
    }
    \label{fig-heatmap_importance_score-sdturbo}
\end{figure}


==> algorithm-figure-table/fig/fig-heatmap_importance_score-sdxl.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{algorithm-figure-table/heatmap_importance_score/sdxl.png}
    \caption{
        Heatmap of importance scores for SDXL. 
    }
    \label{fig-heatmap_importance_score-sdxl}
\end{figure}


==> algorithm-figure-table/fig/fig-heatmap_importance_score-sdxlturbo.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{algorithm-figure-table/heatmap_importance_score/sdxl-turbo.png}
    \caption{
        Heatmap of importance scores for SDXL-Turbo. 
    }
    \label{fig-heatmap_importance_score-sdxlturbo}
\end{figure}


==> algorithm-figure-table/fig/fig-hpd_sdturbo_sdxlturbo_fix_r_appx.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\linewidth]{algorithm-figure-table/hpd_sdturbo_sdxlturbo_fix_r/hpd_sdturbo_sdxlturbo_fix_r.png}
    \caption{
        (Fig.~\ref{fig-hpd_sdturbo_sdxlturbo_fix_r} in the main paper. ) 
        Line chart showing the effect of re-weighting on SD-Turbo and SDXL-Turbo with fixed $high = 1.1$ as $low$ varies. 
        Lines of the same color represent the same category, where dashed lines indicate the vanilla schedule, and solid lines represent our re-weighting schedule. 
    }
    \label{fig-hpd_sdturbo_sdxlturbo_fix_r_appx}
\end{figure}

==> algorithm-figure-table/fig/fig-importance_based_reweighting_sdturbo_appx_1.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c c}
        \hline

        \textbf{Re-Weighting} & \multicolumn{4}{c}{\textbf{SD-Turbo}} \\
        \textbf{Strategy} & anime & concept-art & paintings & photo \\
        
        \hline

        \rule{0pt}{0pt} \\
        
        % Vanilla
        \parbox[t][-2.75cm][c]{2.0cm}{\centering Vanilla} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/default.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/default.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/default.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/default.png} \\

        \rule{0pt}{0pt} \\

        \hdashline

        \rule{0pt}{0pt} \\
            
        % [0.95, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.95, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/0.95_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/0.95_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/0.95_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/0.95_1.1.png} \\

        % [0.96, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.96, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/0.96_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/0.96_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/0.96_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/0.96_1.1.png} \\

        % [0.97, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.97, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/0.97_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/0.97_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/0.97_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/0.97_1.1.png} \\

        % [0.98, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.98, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/0.98_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/0.98_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/0.98_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/0.98_1.1.png} \\

        % [0.99, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.99, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/0.99_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/0.99_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/0.99_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/0.99_1.1.png} \\

        % [1.0, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.0, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/1.0_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/1.0_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/1.0_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/1.0_1.1.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \captionof{figure}{
        Samples synthesized by 2-step-inference SD-Turbo under difference re-weighting schedule. 
    }
    \label{fig-importance_based_reweighting_sdturbo_appx_1}
\end{table*}



==> algorithm-figure-table/fig/fig-importance_based_reweighting_sdturbo_appx_2.tex <==
% importance-based re-weighting, SD-Turbo, 2
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c c}
        \hline

        \textbf{Re-Weighting} & \multicolumn{4}{c}{\textbf{SD-Turbo}} \\
        \textbf{Strategy} & anime & concept-art & paintings & photo \\
        
        \hline

        \rule{0pt}{0pt} \\
        
        % [1.01, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.01, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/1.01_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/1.01_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/1.01_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/1.01_1.1.png} \\

        % [1.02, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.02, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/1.02_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/1.02_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/1.02_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/1.02_1.1.png} \\

        % [1.03, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.03, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/1.03_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/1.03_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/1.03_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/1.03_1.1.png} \\

        % [1.04, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.04, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/1.04_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/1.04_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/1.04_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/1.04_1.1.png} \\

        % [1.05, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.05, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/1.05_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/1.05_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/1.05_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/1.05_1.1.png} \\

        \rule{0pt}{0pt} \\

        \hdashline

        \rule{0pt}{0pt} \\

        % [0.98, 1.15]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.98, 1.15]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/0.98_1.15.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/0.98_1.15.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/0.98_1.15.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/0.98_1.15.png} \\

        % [0.98, 1.2]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.98, 1.2]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/anime/0.98_1.2.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/concept-art/0.98_1.2.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/paintings/0.98_1.2.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sd-turbo/photo/0.98_1.2.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \captionof{figure}{
        Samples synthesized by 2-step-inference SD-Turbo under difference re-weighting schedule (cont.). 
    }
    \label{fig-importance_based_reweighting_sdturbo_appx_2}
\end{table*}



==> algorithm-figure-table/fig/fig-importance_based_reweighting_sdxlturbo_appx_1.tex <==
% importance-based re-weighting, SDXL-Turbo, 1
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c c}
        \hline

        \textbf{Re-Weighting} & \multicolumn{4}{c}{\textbf{SDXL-Turbo}} \\
        \textbf{Strategy} & anime & concept-art & paintings & photo \\
        
        \hline

        \rule{0pt}{0pt} \\
        
        % Vanilla
        \parbox[t][-2.75cm][c]{2.0cm}{\centering Vanilla} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/default.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/default.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/default.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/default.png} \\

        \rule{0pt}{0pt} \\

        \hdashline

        \rule{0pt}{0pt} \\
            
        % [0.95, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.95, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/0.95_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/0.95_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/0.95_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/0.95_1.1.png} \\

        % [0.96, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.96, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/0.96_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/0.96_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/0.96_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/0.96_1.1.png} \\

        % [0.97, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.97, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/0.97_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/0.97_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/0.97_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/0.97_1.1.png} \\

        % [0.98, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.98, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/0.98_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/0.98_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/0.98_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/0.98_1.1.png} \\

        % [0.99, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.99, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/0.99_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/0.99_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/0.99_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/0.99_1.1.png} \\

        % [1.0, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.0, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/1.0_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/1.0_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/1.0_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/1.0_1.1.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \captionof{figure}{
        Samples synthesized by 2-step-inference SD-Turbo under difference re-weighting schedule. 
    }
    \label{fig-importance_based_reweighting_sdxlturbo_appx_1}
\end{table*}



==> algorithm-figure-table/fig/fig-importance_based_reweighting_sdxlturbo_appx_2.tex <==
% importance-based re-weighting, SDXL-Turbo, 2
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c c}
        \hline

        \textbf{Re-Weighting} & \multicolumn{4}{c}{\textbf{SDXL-Turbo}} \\
        \textbf{Strategy} & anime & concept-art & paintings & photo \\
        
        \hline

        \rule{0pt}{0pt} \\
        
        % [1.01, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.01, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/1.01_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/1.01_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/1.01_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/1.01_1.1.png} \\

        % [1.02, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.02, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/1.02_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/1.02_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/1.02_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/1.02_1.1.png} \\

        % [1.03, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.03, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/1.03_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/1.03_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/1.03_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/1.03_1.1.png} \\

        % [1.04, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.04, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/1.04_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/1.04_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/1.04_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/1.04_1.1.png} \\

        % [1.05, 1.1]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[1.05, 1.1]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/1.05_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/1.05_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/1.05_1.1.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/1.05_1.1.png} \\

        \rule{0pt}{0pt} \\

        \hdashline

        \rule{0pt}{0pt} \\

        % [0.95, 1.15]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.95, 1.15]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/0.95_1.15.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/0.95_1.15.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/0.95_1.15.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/0.95_1.15.png} \\

        % [0.95, 1.2]
        \parbox[t][-2.75cm][c]{2.0cm}{\centering $[0.95, 1.2]$} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/anime/0.95_1.2.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/concept-art/0.95_1.2.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/paintings/0.95_1.2.png} & 
        \includegraphics[width=0.15\textwidth]{algorithm-figure-table/importance_based_reweighting/sdxl-turbo/photo/0.95_1.2.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \captionof{figure}{
        Samples synthesized by 2-step-inference SDXL-Turbo under difference re-weighting schedule (cont.). 
    }
    \label{fig-importance_based_reweighting_sdxlturbo_appx_2}
\end{table*}



==> algorithm-figure-table/fig/fig-sample_pruned_sdturbo_fruit_skip_1_a.tex <==
% pruned sampling, SD-Turbo, fruit, vanilla 和 skip-1 baselines
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c | c c c}
        \hline

        \textbf{Strategy Index} & ~ & \textbf{Training Set} & ~ & ~ & \textbf{Test Set} & ~ \\
        
        \hline

        \rule{0pt}{0pt} \\
        
        % Vanilla
        \parbox[t][-2.25cm][c]{2.0cm}{\centering Vanilla} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/default.png} \\

        \rule{0pt}{0pt} \\

        \hline

        \rule{0pt}{0pt} \\

        % a.0
        \parbox[t][-2.25cm][c]{2.0cm}{\centering a.0 / \textbf{b.1}} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/static-0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/static-0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/static-0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/static-0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/static-0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/static-0.png} \\

        % a.1
        \parbox[t][-2.25cm][c]{2.0cm}{\centering a.1 / b.2} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/static-1.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/static-1.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/static-1.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/static-1.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/static-1.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/static-1.png} \\

        % a.2
        \parbox[t][-2.25cm][c]{2.0cm}{\centering a.2} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/static-2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/static-2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/static-2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/static-2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/static-2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/static-2.png} \\

        % a.3
        \parbox[t][-2.25cm][c]{2.0cm}{\centering a.3} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/static-3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/static-3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/static-3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/static-3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/static-3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/static-3.png} \\

        % a.4
        \parbox[t][-2.25cm][c]{2.0cm}{\centering a.4} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/static-4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/static-4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/static-4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/static-4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/static-4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/static-4.png} \\

        % a.5
        \parbox[t][-2.25cm][c]{2.0cm}{\centering a.5} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/static-5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/static-5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/static-5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/static-5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/static-5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/static-5.png} \\

        % a.6
        \parbox[t][-2.25cm][c]{2.0cm}{\centering a.6} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/static-6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/static-6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/static-6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/static-6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/static-6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/static-6.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \captionof{figure}{
        Samples synthesized by Vanilla SD-Turbo U-Net, and U-Net with skipping strategies in group (a).
    }
    \label{fig-sample_pruned_sdturbo_fruit_skip_1_a}
\end{table*}


==> algorithm-figure-table/fig/fig-sample_pruned_sdturbo_fruit_skip_1_b.tex <==
% pruned sampling, SD-Turbo, fruit skip-1 ours
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c | c c c}
        \hline

        \textbf{Strategy Index} & ~ & \textbf{Training Set} & ~ & ~ & \textbf{Test Set} & ~ \\
        
        \hline

        \rule{0pt}{0pt} \\

        % b.0
        \parbox[t][-2.25cm][c]{2.0cm}{\centering b.0} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/skip-1_0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/skip-1_0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/skip-1_0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/skip-1_0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/skip-1_0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/skip-1_0.png} \\

        % b.3
        \parbox[t][-2.25cm][c]{2.0cm}{\centering b.3} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/skip-1_3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/skip-1_3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/skip-1_3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/skip-1_3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/skip-1_3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/skip-1_3.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \captionof{figure}{
        Samples synthesized by U-Net with skipping strategies in group (b).
    }
    \label{fig-sample_pruned_sdturbo_fruit_skip_1_b}
\end{table*}


==> algorithm-figure-table/fig/fig-sample_pruned_sdturbo_fruit_skip_2_c.tex <==
% pruned sampling, SD-Turbo, fruit skip-2 baselines
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c | c c c}
        \hline

        \textbf{Strategy Index} & ~ & \textbf{Training Set} & ~ & ~ & \textbf{Test Set} & ~ \\
        
        \hline

        \rule{0pt}{0pt} \\

        % c.0
        \parbox[t][-2.25cm][c]{2.0cm}{\centering c.0} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/static-0,6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/static-0,6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/static-0,6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/static-0,6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/static-0,6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/static-0,6.png} \\

        % c.1
        \parbox[t][-2.25cm][c]{2.0cm}{\centering c.1} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/static-1,5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/static-1,5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/static-1,5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/static-1,5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/static-1,5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/static-1,5.png} \\

        % c.2
        \parbox[t][-2.25cm][c]{2.0cm}{\centering c.2} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/static-2,4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/static-2,4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/static-2,4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/static-2,4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/static-2,4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/static-2,4.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \captionof{figure}{
        Samples synthesized by U-Net with skipping strategies in group (c).
    }
    \label{fig-sample_pruned_sdturbo_fruit_skip_2_c}
\end{table*}


==> algorithm-figure-table/fig/fig-sample_pruned_sdturbo_fruit_skip_2_d.tex <==
% pruned sampling, SD-Turbo, fruit skip-2 ours
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c | c c c}
        \hline

        \textbf{Strategy Index} & ~ & \textbf{Training Set} & ~ & ~ & \textbf{Test Set} & ~ \\
        
        \hline

        \rule{0pt}{0pt} \\

        % d.0
        \parbox[t][-2.25cm][c]{2.0cm}{\centering d.0} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/skip-2_0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/skip-2_0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/skip-2_0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/skip-2_0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/skip-2_0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/skip-2_0.png} \\

        % d.1
        \parbox[t][-2.25cm][c]{2.0cm}{\centering d.1} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/skip-2_1.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/skip-2_1.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/skip-2_1.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/skip-2_1.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/skip-2_1.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/skip-2_1.png} \\

        % d.2
        \parbox[t][-2.25cm][c]{2.0cm}{\centering d.2} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/skip-2_2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/skip-2_2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/skip-2_2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/skip-2_2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/skip-2_2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/skip-2_2.png} \\

        % d.3
        \parbox[t][-2.25cm][c]{2.0cm}{\centering d.3} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/skip-2_3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/skip-2_3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/skip-2_3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/skip-2_3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/skip-2_3.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/skip-2_3.png} \\

        % d.4
        \parbox[t][-2.25cm][c]{2.0cm}{\centering d.4} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/skip-2_4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/skip-2_4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/skip-2_4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/skip-2_4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/skip-2_4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/skip-2_4.png} \\

        % d.5
        \parbox[t][-2.25cm][c]{2.0cm}{\centering d.5} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/skip-2_5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/skip-2_5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/skip-2_5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/skip-2_5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/skip-2_5.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/skip-2_5.png} \\

        % d.6
        \parbox[t][-2.25cm][c]{2.0cm}{\centering d.6} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/skip-2_6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/skip-2_6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/skip-2_6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/skip-2_6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/skip-2_6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/skip-2_6.png} \\

        % d.7
        \parbox[t][-2.25cm][c]{2.0cm}{\centering \textbf{d.7}} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/skip-2_7.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/skip-2_7.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/skip-2_7.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/skip-2_7.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/skip-2_7.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/skip-2_7.png} \\

        % d.8
        \parbox[t][-2.25cm][c]{2.0cm}{\centering d.8} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/23/skip-2_8.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/52/skip-2_8.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/training/74/skip-2_8.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/22/skip-2_8.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/73/skip-2_8.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_pruned/test/83/skip-2_8.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \captionof{figure}{
        Samples synthesized by U-Net with skipping strategies in group (d).
    }
    \label{fig-sample_pruned_sdturbo_fruit_skip_2_d}
\end{table*}


==> algorithm-figure-table/fig/fig-sample_scheduled_sdturbo_astronaunt.tex <==
% 表: importance-uncertainty 加权, SD-Turbo, astronaut, 不同 lam, 不同 high_weight
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c  c c c}
        \hline

        \textbf{Weight} & \multicolumn{6}{c}{$\eta$ \textbf{values}} \\
        \textbf{Range} & 0.0 & 0.2 & 0.4 & 0.6 & 0.8 & 1.0 \\
        
        \hline

        \rule{0pt}{0pt} \\
        
        % high_weight: 1.05
        \parbox[t][-2.25cm][c]{2.0cm}{\centering $[0.98, 1.05]$} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.05/lam-0.0.png} &
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.05/lam-0.2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.05/lam-0.4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.05/lam-0.6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.05/lam-0.8.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.05/lam-1.0.png} \\ 
    
        % high_weight: 1.08
        \parbox[t][-2.25cm][c]{2.0cm}{\centering $[0.98, 1.08]$} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.08/lam-0.0.png} &
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.08/lam-0.2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.08/lam-0.4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.08/lam-0.6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.08/lam-0.8.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.08/lam-1.0.png} \\
    
        % high_weight: 1.1
        \parbox[t][-2.25cm][c]{2.0cm}{\centering $[0.98, 1.1]$} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.1/lam-0.0.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.1/lam-0.2.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.1/lam-0.4.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.1/lam-0.6.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.1/lam-0.8.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/high_weight-1.1/lam-1.0.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \caption{
        Samples evolve across various weight range and $\eta$ values. 
    }
    \label{fig-sample_scheduled_sdturbo_astronaunt}
\end{table*}



==> algorithm-figure-table/fig/fig-sample_scheduled_sdturbo_bear_failure.tex <==
% 表: importance-uncertainty 加权, SD-Turbo, astronaut, 不同 lam, 不同 high_weight
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c  c c c}
        \hline

        \textbf{Standard} & \multicolumn{6}{c}{$\eta$ \textbf{values}} \\
        \textbf{SD-Turbo} & 0.0 & 0.2 & 0.4 & 0.6 & 0.8 & 1.0 \\
        
        \hline

        \rule{0pt}{0pt} \\

        % with detail
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_bear_failure/standard_detail.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_bear_failure/lam-0.0_detail.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_bear_failure/lam-0.2_detail.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_bear_failure/lam-0.4_detail.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_bear_failure/lam-0.6_detail.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_bear_failure/lam-0.8_detail.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_scheduled_sdturbo_bear_failure/lam-1.0_detail.png} \\
        
        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \caption{
        A failure case of our enhanced image synthesis. 
        Key regions of great difference are highlighted with blue rectangles. 
    }
    \label{fig-sample_scheduled_sdturbo_bear_failure}
\end{table*}



==> algorithm-figure-table/fig/fig-sample_scheduled_sdturbo_dog.tex <==
% 表: 不同跳过策略下的 SD-Turbo, dog
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c c c}
        \hline
        
        \multirow{2}{*}{\textbf{Vanilla}} & \multicolumn{5}{c}{\textbf{Skipping Strategy Index}} \\
        
        ~ & a.0 / b.2 & a.1 & b.0 & f.1 & g.4 \\
        
        \hline

        \rule{0pt}{0pt} \\

        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_pruning-sdturbo-dog/vanilla.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_pruning-sdturbo-dog/a.0.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_pruning-sdturbo-dog/a.1.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_pruning-sdturbo-dog/b.0.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_pruning-sdturbo-dog/f.1.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_pruning-sdturbo-dog/g.4.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}

    \caption{
        Samples from the test set with skipping strategies in Tab.~\ref{tab-skipping_strategy_sdturbo_dog_selected}. 
        Only the strategies with best FID in training set or test set in each group are displayed. 
        Images are evaluated at $512^2$ px.
    }
    \label{fig-sample_scheduled_sdturbo_dog}
\end{table*}

==> algorithm-figure-table/fig/fig-sample_standard_sdturbo_astronaut.tex <==
\begin{figure}[t]
    \centering

    \includegraphics[width=0.5\linewidth]{algorithm-figure-table/sample_scheduled_sdturbo_astronaut/standard.png}
    \caption{
        Sample generated with standard SD-Turbo. 
    }
    \label{fig-sample_standard_sdturbo_astronaut}
\end{figure}


==> algorithm-figure-table/fig/fig-scatter_fid_lpips_fruit_appx.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\linewidth]{algorithm-figure-table/scatter_fid_lpips/scatter_fid_lpips_fruit.png}
    \caption{
        (Fig.~\ref{fig-scatter_fid_lpips_fruit} in the main paper)
        Scatter plot of FID and LPIPS under different skipping strategies (the further lower-left, the better). 
        Baseline strategies are represented by blue circles, unique points from our strategies are shown as pink triangles, while points overlapping with baseline points are marked with purple stars.
    }
    \label{fig-scatter_fid_lpips_fruit_appx}
    \vspace{-10pt}
\end{figure}

==> algorithm-figure-table/fig/fig-source_image_ddim_inversion.tex <==
\begin{figure}[t]
    \centering

    \includegraphics[width=0.5\linewidth]{algorithm-figure-table/ddim_inversion_lam_zjh/source_detail.png}
    \caption{
        Source image for DDIM Inversion. 
        Key areas are zoomed in and displayed in the chartreuse and red rectangles.  
    }
    \label{fig-source_image_ddim_inversion}
\end{figure}


==> algorithm-figure-table/fig/fig-static_reweighting_sd_sdxl_appx.tex <==
% SD / SDXL static re-weighting 的采样图
\begin{table*}[h]
    \centering
    \begin{tabular}{c | c c c | c c c}
        \hline

        \textbf{Re-Weighting} & \multicolumn{3}{c|}{\textbf{SD v2.1}} & \multicolumn{3}{c}{\textbf{SDXL}} \\
        \textbf{Strategy} & 10-step & 15-step & 20-step & 10-step & 15-step & 20-step \\
        
        \hline

        \rule{0pt}{0pt} \\
        
        % default
        \parbox[t][-2.25cm][c]{2.0cm}{\centering Vanilla} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd/10_step/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd/15_step/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd/20_step/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl/10_step/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl/15_step/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl/20_step/default.png} \\
        
        % ours
        \parbox[t][-2.25cm][c]{2.0cm}{\centering Vanilla} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd/10_step/ours.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd/15_step/ours.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd/20_step/ours.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl/10_step/ours.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl/15_step/ours.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl/20_step/ours.png} \\
        
        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \captionof{figure}{
        Samples of SD and SDXL with different inference steps, using the vanilla re-weighting schedule and our best re-weighting schedule, respectively. 
    }
    \label{fig-static_reweighting_sd_sdxl_appx}
\end{table*}



==> algorithm-figure-table/fig/fig-static_reweighting_sdturbo_sdxlturbo_appx.tex <==
% SD-Turbo / SDXL-Turbo, static re-weighting 的采样图
\begin{table*}[h]
    \centering
    \begin{tabular}{c | c c c | c c c}
        \hline

        \textbf{Re-Weighting} & \multicolumn{3}{c|}{\textbf{SD-Turbo}} & \multicolumn{3}{c}{\textbf{SDXL-Turbo}} \\
        \textbf{Strategy} & 1-step & 2-step & 3-step & 1-step & 2-step & 3-step \\
        
        \hline

        \rule{0pt}{0pt} \\
        
        % default
        \parbox[t][-2.25cm][c]{2.0cm}{\centering Vanilla} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd-turbo/1_step/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd-turbo/2_step/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd-turbo/3_step/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl-turbo/1_step/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl-turbo/2_step/default.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl-turbo/3_step/default.png} \\
        
        % ours
        \parbox[t][-2.25cm][c]{2.0cm}{\centering Vanilla} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd-turbo/1_step/ours.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd-turbo/2_step/ours.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sd-turbo/3_step/ours.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl-turbo/1_step/ours.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl-turbo/2_step/ours.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/static_reweighting/sdxl-turbo/3_step/ours.png}
        \rule{0pt}{0pt} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}
    \captionof{figure}{
        Samples of SD-Turbo and SDXL-Turbo with different inference steps, using the vanilla re-weighting schedule and our best re-weighting schedule, respectively. 
    }
    \label{fig-static_reweighting_sdturbo_sdxlturbo_appx}
\end{table*}



==> algorithm-figure-table/fig/fig-weighted_u_net_appx.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\linewidth]{algorithm-figure-table/fig/weighted_U-Net_bg_floor.png}
    \caption{
        (Fig. 1 in the main paper) 
        Schematic of scaling the outputs of seven Transformer blocks before passing to the subsequent ResNet~\cite{he2016deep} blocks. 
        The blue rectangles represent the ResNet blocks, while the pink ones stand for the Transformer blocks. 
    }
    \label{fig-weighted_u_net_appx}
\end{figure}


==> algorithm-figure-table/tab/tab-comparison_between_differnt_step_appx.tex <==
% 双栏
\begin{table*}[t]
    \caption{
        (Tab.~\ref{tab-comparison_between_different_models_and_steps} in the main paper) 
        Comparison between different models and inference steps. 
        Cells with a red/orange/yellow background indicate the best/second-best/third-best performance, respectively.  
        Cells where the weighted performance is worse than the vanilla schedule are marked with a downward arrow $\downarrow$. 
        Blocks within the SD/SDXL family are numbered from 0/1 for symmetry. 
    }
    \centering
    \begin{tabular}{c | c c c : c c c | c c c : c c c}
        \hline
        \multirow{2}{*}{\textbf{Weighting}} &
        \multicolumn{3}{c:}{\textbf{SD-Turbo}} & 
        \multicolumn{3}{c|}{\textbf{SDXL-Turbo}} & 
        \multicolumn{3}{c:}{\textbf{SD v2.1}} & 
        \multicolumn{3}{c}{\textbf{SDXL}} \\
        ~ & 1 & 2 & 3 & 1 & 2 & 3 &
        10 & 15 & 20 & 10 & 15 & 20 \\

        \hline
        Vanilla & 
        0.2961 & 0.3059 & 0.3034 & 
        0.2587 & 0.2693 & 0.2666 & 
        0.2876 & 0.2908 & 0.2932 & 
        0.2830 & \tbest{0.2889} & \tbest{0.2904} \\

        \hdashline

        blk-0 & 
        \sbest{0.2987} & \best{0.3088} & \tbest{0.3045} & 
        / & / & / & 
        0.2860$\downarrow$ & 0.2915 & \sbest{0.2946} & 
        / & / & / \\
        
        blk-1 & 
        \best{0.2993} & 0.3066 & 0.3019$\downarrow$ & 
        \best{0.2591} & 0.2685$\downarrow$ & 0.2666 & 
        \tbest{0.2881} & 0.2908 & \tbest{0.2943} & 
        \sbest{0.2863} & \best{0.2907} & \best{0.2924} \\
        
        blk-2 & 
        0.2966 & 0.3065 & 0.3037 & 
        0.2584$\downarrow$ & 0.2686$\downarrow$ & 0.2661$\downarrow$ & 
        0.2880 & 0.2896$\downarrow$ & 0.2935 & 
        0.2842 & 0.2886$\downarrow$ & 0.2889$\downarrow$ \\
        
        blk-3 & 
        0.2962 & 0.3055$\downarrow$ & 0.3035 & 
        \sbest{0.2589} & \best{0.2697} & \tbest{0.2668} & 
        0.2876 & 0.2909 & 0.2934 & 
        0.2839 & 0.2877$\downarrow$ & 0.2898$\downarrow$ \\
        
        blk-4 & 
        0.2965 & \sbest{0.3074} & \sbest{0.3052} & 
        \tbest{0.2588} & \sbest{0.2695} & \best{0.2671} & 
        \sbest{0.2894} & \tbest{0.2917} & 0.2939 & 
        \tbest{0.2851} & \tbest{0.2889} & 0.2892$\downarrow$ \\
        
        blk-5 & 
        \tbest{0.2981} & 0.3066 & \best{0.3062} & 
        0.2576$\downarrow$ & \tbest{0.2694} & \sbest{0.2670} & 
        \best{0.2902} & \best{0.2923} & \best{0.2950} & 
        \best{0.2868} & \sbest{0.2904} & \best{0.2910} \\
        
        blk-6 & 
        0.2962 & \tbest{0.3072} & 0.3025$\downarrow$ & 
        / & / & / & 
        0.2880 & \sbest{0.2919} & 0.2927$\downarrow$ & 
        / & / & / \\
        
        \hline
    \end{tabular}
    \label{tab-comparison_between_different_models_and_steps_appx}
\end{table*}


==> algorithm-figure-table/tab/tab-fid_lpips_fruit_all_appx.tex <==
% SD-Turbo 跳过策略 (全)
\begin{table}[h]
    \centering
    \begin{tabular}{c | c c : c c}
        \hline
        
        \textbf{Strategy} & \multicolumn{2}{c:}{\textbf{FID} $\downarrow$} & \multicolumn{2}{c}{\textbf{LPIPS} $\downarrow$} \\
        
        \textbf{Index} & train & test & train & test \\
        
        \hline

        % skip-1: baseline
        a.0 / \textbf{b.1} & 402.8469 & 397.1920 & 0.7148 & 0.6894 \\
        a.1 / b.2 & 241.3091 & 244.8477 & \sbest{0.6170} & 0.6201 \\
        a.2 & \sbest{176.8128} & \sbest{173.6468}  & \tbest{0.6309} & 0.6274 \\
        a.3 & \best{40.4357} & \best{39.7413} & \best{0.3915} & \best{0.5266} \\
        a.4 & \tbest{215.3175} & \tbest{214.6077}  & 0.6350 & \sbest{0.5603} \\
        a.5 & 242.5459 & 240.0058  & 0.6334 & \tbest{0.5763} \\
        a.6 & 401.0944 & 404.0254  & 0.8366 & 0.8085 \\

        \hdashline

        % skip-1: ours
        b.0 & 354.4077 & 356.5143  & 0.6550 & 0.6509 \\
        % b.1 & ~ & ~ \\
        % b.2 & ~ & ~ \\
        b.3 & 259.9984 & 259.2821  & 0.6439 & 0.6293 \\

        \hline

        % skip-2: baseline
        c.0 & 453.6726 & 456.1274  & 0.8295 & 0.8302 \\
        c.1 & 401.6146 & 401.9952  & \sbest{0.6595} & \best{0.6436} \\
        c.2 & 362.4762 & 357.4724  & \best{0.6513} & \sbest{0.6623} \\

        \hdashline

        % skip-2: ours
        d.0 & 457.7766 & 456.3885  & 0.6959 & 0.6964 \\
        d.1 & 467.9547 & 464.4429  & 0.7593 & 0.7642 \\
        d.2 & 472.7829 & 466.7573  & 0.8131 & 0.8022 \\
        d.3 & 409.4545 & 412.3269  & \tbest{0.6853} & \tbest{0.6822} \\
        d.4 & 371.9738 & 387.3718  & 0.7331 & 0.7514 \\
        d.5 & 374.8360 & 383.1508  & 0.7815 & 0.7822 \\
        d.6 & \tbest{313.1157} & \tbest{309.0396}  & 0.7194 & 0.7149 \\
        \textbf{d.7} & \best{305.8840} & \best{304.8817} & 0.7048 & 0.7084 \\
        d.8 & \sbest{307.3236} & \sbest{304.9316}  & 0.7339 & 0.7067 \\

        \hline
    \end{tabular}
    \caption{
        Comparison of FID and LPIPS between vanilla, baseline skipping strategies, and our suggested strategies. 
        Multiple skipping strategies between adjacent solid or dashed lines are grouped as one set. 
    }
    \label{tab-fid_lpips_fruit_all_appx}
\end{table}

==> algorithm-figure-table/tab/tab-hpd_sdturbo_sdxlturbo_seleceted_appx.tex <==
% SD-Turbo/SDXL-Turbo 加权 (selected) (单栏)
\begin{minipage}{1.035\columnwidth}
    \centering
    
    % SD-Turbo 加权 (selected)
    \captionof{table}{
        (Tab.~\ref{tab-hpd_sdturbo_selected} in the main paper) 
        Enhanced SD-Turbo (selected). 
    }
    \label{tab-hpd_sdturbo_selected_appx}
    \hspace{-3em}
    \resizebox{0.98\columnwidth}{!}{
        % \begin{table}[h]
        \centering
        \begin{tabular}{c | c c c c c c c c | c c}
            \hline
            \multirow{2}{*}{\textbf{Weighting}} &
            \multicolumn{2}{c}{\textbf{anime}} & 
            \multicolumn{2}{c}{\textbf{concept-art}} & 
            \multicolumn{2}{c}{\textbf{paintings}} & 
            \multicolumn{2}{c|}{\textbf{photo}} &
            \multicolumn{2}{c}{\textbf{avg}} \\
    
            ~ & 
            train & test & train & test &
            train & test & train & test & 
            train & test \\
    
            \hline

            Vanilla & 
            0.2826 & 0.2849 &
            0.2763 & 0.2787 &
            0.2788 & 0.2801 &
            0.2814 & 0.2806 & 
            0.2798 & 0.2811 \\

            \hdashline

            $[0.98, 1.1]$ & 
             \best{0.2863} & \sbest{0.2881} & 
             \best{0.2798} & \best{0.2833} &
             \sbest{0.2834} & \best{0.2842} &
             \sbest{0.2851} & \sbest{0.2848} & 
             \best{0.2837} & \best{0.2851} \\

             $[1.02, 1.1]$ & 
             \sbest{0.2860} & \best{0.2883} & 
             \sbest{0.2796} & \sbest{0.2828} &
             \best{0.2836} & \sbest{0.2840} &
             \best{0.2854} & \best{0.2849} & 
             \best{0.2837} & \sbest{0.2850} \\

            \hdashline

            $[0.98, 1.15]$ & 
             \tbest{0.2859} & \tbest{0.2875} & 
             \tbest{0.2793} & \tbest{0.2822} &
             \tbest{0.2833} & \tbest{0.2839} &
             \tbest{0.2845} & \tbest{0.2840} & 
             \sbest{0.2833} & \tbest{0.2844} \\

             $[1.02, 1.15]$ & 
             0.2853 & 0.2869 & 
             0.2783 & 0.2809 &
             0.2822 & 0.2832 &
             0.2843 & 0.2830 & 
             \tbest{0.2825} & 0.2835 \\

             \hdashline

             $[0.98, 1.2]$ & 
             0.2852 & 0.2860 & 
             0.2776 & 0.2802 &
             0.2815 & 0.2823 &
             0.2828 & 0.2815 & 
             0.2818 & 0.2825 \\

             $[1.02, 1.2]$ & 
             0.2833 & 0.2837 & 
             0.2758 & 0.2786 &
             0.2802 & 0.2809 &
             0.2815 & 0.2794 & 
             0.2802 & 0.2806 \\

            \hline
        \end{tabular}
    }

    % SDXL-Turbo 加权 (selected)
    \captionof{table}{
        (Tab.~\ref{tab-hpd_sdxlturbo_selected} in the main paper) 
        Enhanced SDXL-Turbo (selected). 
    }
    \label{tab-hpd_sdxlturbo_selected_appx}
    \hspace{-3em}
    \resizebox{0.98\columnwidth}{!}{
        % \begin{table}[h]
        \centering
        \begin{tabular}{c | c c c c c c c c | c c}
            \hline
            \multirow{2}{*}{\textbf{Weighting}} &
            \multicolumn{2}{c}{\textbf{anime}} & 
            \multicolumn{2}{c}{\textbf{concept-art}} & 
            \multicolumn{2}{c}{\textbf{paintings}} & 
            \multicolumn{2}{c|}{\textbf{photo}} &
            \multicolumn{2}{c}{\textbf{avg}} \\
    
            ~ & 
            train & test & train & test &
            train & test & train & test & 
            train & test \\
    
            \hline

            Vanilla & 
            \tbest{0.2848} & 0.2898 &
            \tbest{0.2785} & 0.2815 &
            \tbest{0.2785} & \tbest{0.2812} &
            \tbest{0.2804} & \tbest{0.2818} & 
            \tbest{0.2801} & 0.2836 \\

            \hdashline

            $[0.95, 1.1]$ & 
             \best{0.2881} & \tbest{0.2910} & 
             \best{0.2814} & \sbest{0.2842} &
             \best{0.2819} & \best{0.2847} &
             \best{0.2833} & \sbest{0.2847} & 
             \best{0.2837} & \sbest{0.2862} \\

            $[0.95, 1.15]$ & 
             \best{0.2881} & \best{0.2923} & 
             \best{0.2814} & \best{0.2844} &
             \sbest{0.2818} & \sbest{0.2844} &
             \best{0.2833} & \best{0.2848} & 
             \best{0.2837} & \best{0.2865} \\

             $[0.95, 1.2]$ & 
             \sbest{0.2878} & \sbest{0.2916} & 
             \sbest{0.2810} & \tbest{0.2838} &
             \best{0.2816} & \best{0.2839} &
             \sbest{0.2826} & \best{0.2842} & 
             \sbest{0.2832} & \tbest{0.2859} \\
        
            \hline
        \end{tabular}
    }
\end{minipage}


==> algorithm-figure-table/tab/tab-hyper_parameter_weight_threshold_update_schedule.tex <==
\begin{table}[h]
    \centering
    \caption{
        Hyper-parameters for the Weight Threshold Update Schedule. 
    }
    \begin{tabular}{c | c}
        \hline
        Param Name & Value \\
        \hline

        $\epsilon$ & $1\text{e}-2$ \\

        \hdashline

        $P(B_1 \mid A)$ & $0.06$ \\
        $P_{\text{st}} (B_2 \mid A)$ & $0.47$ \\ 
        $P_{\text{ed}} (B_2 \mid A)$ & $0.84$ \\ 
        $P_{\text{st}} (B_3 \mid A)$ & $0.47$ \\ 
        $P_{\text{ed}} (B_3 \mid A)$ & $0.10$ \\ 

        \hdashline

        $P_{\text{st}} (B_1 \mid \overline{A})$ & $0.48$ \\ 
        $P_{\text{ed}} (B_1 \mid \overline{A})$ & $0.30$ \\ 
        $P_{\text{st}} (B_2 \mid \overline{A})$ & $0.48$ \\ 
        $P_{\text{ed}} (B_2 \mid \overline{A})$ & $0.66$ \\ 
        
        $P(B_3 \mid \overline{A})$ & $0.04$ \\ 

        \hline
    \end{tabular}
    \label{tab-hyper_parameter_weight_threshold_update_schedule}
\end{table}

==> algorithm-figure-table/tab/tab-importance_sd_sdxl_fruit_appx.tex <==
\begin{table}[h]
    \centering
    \caption{
        Dynamic importance ranking of 20-step SD v2.1/SDXL U-Net, arranged in non-descending order. 
    }
    \begin{tabular}{c | c : c}
        \hline
        \multirow{2}{*}{\textbf{Step}} & 
        \multicolumn{2}{c}{\textbf{Importance Ranking}} \\

        ~ & SD v2.1 & SDXL \\
        \hline

        0 & 6 2 3 0 4 1 5 & 5 4 2 3 1 \\ 
        1 & 0 2 6 4 5 3 1 & 3 4 2 1 5 \\  
        2 & 6 5 1 0 2 4 3 & 1 5 2 3 4 \\  
        3 & 0 2 6 1 5 3 4 & 5 4 3 1 2 \\  
        4 & 0 6 5 1 3 4 2 & 4 5 1 2 3 \\  
        5 & 0 1 2 6 3 5 4 & 5 1 3 2 4 \\  
        6 & 0 5 4 3 1 6 2 & 5 1 4 3 2 \\  
        7 & 0 5 6 4 1 3 2 & 1 5 4 2 3 \\  
        8 & 0 5 6 1 2 4 3 & 5 1 4 3 2 \\  
        9 & 0 1 6 2 5 4 3 & 5 1 4 3 2 \\  
        10 & 0 6 1 5 2 4 3 & 5 1 4 3 2 \\  
        11 & 0 1 5 6 4 3 2 & 5 1 4 2 3 \\  
        12 & 0 5 4 6 1 2 3 & 5 1 3 2 4 \\  
        13 & 5 0 6 4 1 2 3 & 5 1 4 3 2 \\  
        14 & 0 5 6 4 1 2 3 & 5 1 2 4 3 \\  
        15 & 6 0 5 1 4 2 3 & 5 1 4 3 2 \\  
        16 & 0 5 6 1 2 4 3 & 5 1 4 3 2 \\  
        17 & 6 0 5 2 1 4 3 & 5 1 4 2 3 \\  
        18 & 0 5 6 1 3 4 2 & 5 1 4 2 3 \\  
        19 & 5 6 0 1 2 3 4 & 5 1 4 2 3 \\  
        
        \hline
    \end{tabular}
    \label{tab-importance_sd_sdxl_fruit_appx}
\end{table}

==> algorithm-figure-table/tab/tab-importance_sdturbo_sdxlturbo_fruit_appx.tex <==
\begin{table}[h]
    \centering
    \caption{
        (Tab.~\ref{tab-dynamic_importance_ranking_fruit} in the main paper) 
        Dynamic importance ranking of 2-step SD-Turbo/SDXL-Turbo U-Net, arranged in non-descending order. 
    }
    \begin{tabular}{c | c : c}
        \hline
        \multirow{2}{*}{\textbf{Step}} & 
        \multicolumn{2}{c}{\textbf{Importance Ranking}} \\

        ~ & SD-Turbo & SDXL-Turbo \\
        \hline

        0 & 0 1 2 4 6 5 3 & 1 2 5 3 4 \\ 
        1 & 1 0 5 4 2 6 3 & 1 2 5 4 3 \\ 

        \hline
    \end{tabular}
    \label{tab-importance_sdturbo_sdxlturbo_fruit_appx}
\end{table}

==> algorithm-figure-table/tab/tab-sample_scheduled_ddim_inversion_kitten_cjl.tex <==
% 表: 分别对不同 block 作固定加权, DDIM Inversion, kitten_cjl
\begin{table*}[t]
    \centering
    
    \begin{tabular}{c | c c c c c c}
        \hline
        
        \textbf{Input} & \textbf{block-0} & \textbf{block-1} & \textbf{block-2} & \textbf{block-3} & \textbf{block-4} & \textbf{block-5} \\
        
        \hline

        \rule{0pt}{0pt} \\

        % w detail
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/ddim_inversion_lam_zjh/standard.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/lam-0.0_detail.png} & 
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/lam-0.25_detail.png} &
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/lam-0.5_detail.png} &
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/lam-0.0_detail.png} &
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/lam-0.25_detail.png} &
        \includegraphics[width=0.12\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/lam-0.5_detail.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}

    \caption{
        \TODO{replace the figures}
    }
    \label{tab-sample_scheduled_ddim_inversion_kitten_cjl}
\end{table*}


==> algorithm-figure-table/tab/tab-sample_scheduled_ddim_inversion_zjh.tex <==
% 表: 不同 lambda 下, importance-uncertainty 加权, DDIM Inversion, zjh
\begin{table*}[t]
    \centering
    \begin{tabular}{c c c c c c}
        \hline
        
        \multicolumn{6}{c}{$\eta$ \textbf{of Hybrid Score}} \\
        
        0.0 & 0.2 & 0.4 & 0.6 & 0.8 & 1.0 \\
        
        \hline

        \rule{0pt}{0pt} \\

        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/ddim_inversion_lam_zjh/nudging-1.025/lam-0.0_nudging-1.025.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/ddim_inversion_lam_zjh/nudging-1.025/lam-0.2_nudging-1.025.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/ddim_inversion_lam_zjh/nudging-1.025/lam-0.4_nudging-1.025.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/ddim_inversion_lam_zjh/nudging-1.025/lam-0.6_nudging-1.025.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/ddim_inversion_lam_zjh/nudging-1.025/lam-0.8_nudging-1.025.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/ddim_inversion_lam_zjh/nudging-1.025/lam-1.0_nudging-1.025.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}

    \caption{
        Differences in detail preservation in non-focal areas under different $\eta$ values. 
    }
    \label{tab-sample_scheduled_ddim_inversion_zjh}
\end{table*}


==> algorithm-figure-table/tab/tab-sample_scheduled_sdturbo_bear.tex <==
% 表: 不同 lambda 下, importance-uncertainty 加权, SD-Turbo, bear
\begin{table*}[t]
    \centering
    \begin{tabular}{c | c c c c c}
        \hline
        
        \multirow{2}{*}{}{\textbf{Vanilla}} & \multicolumn{5}{c}{$\eta$ \textbf{of Hybrid Score}} \\
        
        \textbf{SD-Turbo (2 steps)} & 0.0 & 0.25 & 0.5 & 0.75 & 1.0 \\
        
        \hline

        \rule{0pt}{0pt} \\

        % w detail
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/vanilla_detail.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/lam-0.0_detail.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/lam-0.25_detail.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/lam-0.5_detail.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/lam-0.75_detail.png} & 
        \includegraphics[width=0.14\textwidth]{algorithm-figure-table/sample_lam_sdturbo_bear/lam-1.0_detail.png} \\

        \rule{0pt}{0pt} \\

        \hline
    \end{tabular}

    \caption{
        Visual quality enhancement with hybrid score under different $\eta$ values. 
        Regions with noticeable differences in detail level are highlighted with pink rectangles. 
        Unless otherwise specified, all images in this work are evaluated at $512^2$ px.
    }
    \label{tab-sample_scheduled_sdturbo_bear}
\end{table*}

==> algorithm-figure-table/tab/tab-sd_turbo_best_ablation.tex <==
% SD-Turbo 加权 [0.98, 11], 重要性得分逆序 (单栏)
\begin{minipage}{1.035\columnwidth}
    \centering
    \captionof{table}{
        SD-Turbo Ablation. 
    }
    \hspace{-3em}
    \resizebox{0.98\columnwidth}{!}{
        \centering
        \begin{tabular}{c | c c c c c c c c | c c}
            \hline
            \multirow{2}{*}{\textbf{Weighting}} &
            \multicolumn{2}{c}{\textbf{anime}} & 
            \multicolumn{2}{c}{\textbf{concept-art}} & 
            \multicolumn{2}{c}{\textbf{paintings}} & 
            \multicolumn{2}{c|}{\textbf{photo}} &
            \multicolumn{2}{c}{\textbf{avg}} \\
    
            ~ & 
            train & test & train & test &
            train & test & train & test & 
            train & test \\
    
            \hline

            Vanilla & 
            0.2826 & 0.2849 &
            0.2763 & 0.2787 &
            0.2788 & \sbest{0.2801} &
            0.2814 & 0.2806 & 
            0.2798 & \sbest{0.2811} \\

            \hdashline

            $[0.98, 1.1]^{\text{rev}}$ & 
            \sbest{0.2857} & \best{0.2885} & 
            \sbest{0.2789} & \sbest{0.2826} &
            \sbest{0.2831} & \best{0.2842} &
            \best{0.2857} & \best{0.2853} & 
            \sbest{0.2834} & \best{0.2851} \\

            $[0.98, 1.1]$ & 
            \best{0.2863} & \sbest{0.2881} & 
            \best{0.2798} & \best{0.2833} &
            \best{0.2834} & \best{0.2842} &
            \sbest{0.2851} & \sbest{0.2848} & 
            \best{0.2837} & \best{0.2851} \\

            \hline
        \end{tabular}
        
    }
    \label{tab-sd_turbo_best_ablation}
\end{minipage}


==> algorithm-figure-table/tab/tab-sd_turbo_fix_l.tex <==
% SD-Turbo 加权 [0.98, ?], [1.02, ?] (单栏)
\begin{minipage}{1.035\columnwidth}
    \centering
    \captionof{table}{
        Enhanced SD-Turbo ($l = 0.98, 1.02$). 
    }
    \hspace{-3em}
    \resizebox{0.98\columnwidth}{!}{
        \centering
        \begin{tabular}{c | c c c c c c c c | c c}
            \hline
            \multirow{2}{*}{\textbf{Weighting}} &
            \multicolumn{2}{c}{\textbf{anime}} & 
            \multicolumn{2}{c}{\textbf{concept-art}} & 
            \multicolumn{2}{c}{\textbf{paintings}} & 
            \multicolumn{2}{c|}{\textbf{photo}} &
            \multicolumn{2}{c}{\textbf{avg}} \\
    
            ~ & 
            train & test & train & test &
            train & test & train & test & 
            train & test \\
    
            \hline

            Vanilla & 
            0.2826 & 0.2849 &
            0.2763 & 0.2787 &
            0.2788 & 0.2801 &
            0.2814 & 0.2806 & 
            0.2798 & 0.2811 \\

            \hdashline

            $[0.98, 1.1]$ & 
             \best{0.2863} & \sbest{0.2881} & 
             \best{0.2798} & \best{0.2833} &
             \sbest{0.2834} & \best{0.2842} &
             \sbest{0.2851} & \sbest{0.2848} & 
             \best{0.2837} & \best{0.2851} \\

             $[1.02, 1.1]$ & 
             \sbest{0.2860} & \best{0.2883} & 
             \sbest{0.2796} & \sbest{0.2828} &
             \best{0.2836} & \sbest{0.2840} &
             \best{0.2854} & \best{0.2849} & 
             \best{0.2837} & \sbest{0.2850} \\

            \hdashline

            $[0.98, 1.15]$ & 
             \tbest{0.2859} & \tbest{0.2875} & 
             \tbest{0.2793} & \tbest{0.2822} &
             \tbest{0.2833} & \tbest{0.2839} &
             \tbest{0.2845} & \tbest{0.2840} & 
             \sbest{0.2833} & \tbest{0.2844} \\

             $[1.02, 1.15]$ & 
             0.2853 & 0.2869 & 
             0.2783 & 0.2809 &
             0.2822 & 0.2832 &
             0.2843 & 0.2830 & 
             \tbest{0.2825} & 0.2835 \\

             \hdashline

             $[0.98, 1.2]$ & 
             0.2852 & 0.2860 & 
             0.2776 & 0.2802 &
             0.2815 & 0.2823 &
             0.2828 & 0.2815 & 
             0.2818 & 0.2825 \\

             $[1.02, 1.2]$ & 
             0.2833 & 0.2837 & 
             0.2758 & 0.2786 &
             0.2802 & 0.2809 &
             0.2815 & 0.2794 & 
             0.2802 & 0.2806 \\

        
            \hline
        \end{tabular}
        
    }
    \label{tab-sd_turbo_fix_l}
\end{minipage}


==> algorithm-figure-table/tab/tab-sd_turbo_fix_r.tex <==
% SD-Turbo 加权 [?, 1.1] (单栏)
\begin{minipage}{1.035\columnwidth}
    \centering
    \captionof{table}{
        Enhanced SD-Turbo ($r = 1.1$). 
    }
    \hspace{-3em}
    \resizebox{0.98\columnwidth}{!}{
        \centering
        \begin{tabular}{c | c c c c c c c c | c c}
            \hline
            \multirow{2}{*}{\textbf{Weighting}} &
            \multicolumn{2}{c}{\textbf{anime}} & 
            \multicolumn{2}{c}{\textbf{concept-art}} & 
            \multicolumn{2}{c}{\textbf{paintings}} & 
            \multicolumn{2}{c|}{\textbf{photo}} &
            \multicolumn{2}{c}{\textbf{avg}} \\
    
            ~ & 
            train & test & train & test &
            train & test & train & test & 
            train & test \\
    
            \hline

            Vanilla & 
            0.2826 & 0.2849 &
            0.2763 & 0.2787 &
            0.2788 & 0.2801 &
            0.2814 & 0.2806 & 
            0.2798 & 0.2811 \\

            \hdashline

            $[0.95, 1.1]$ & 
            0.2856 & 0.2879 & 
            \best{0.2814} & 0.2829 &
            0.2827 & \tbest{0.2843} &
            0.2841 & 0.2839 & 
            0.2834 & 0.2847 \\

            $[0.96, 1.1]$ & 
             0.2858 & 0.2879 & 
             0.2792 & 0.2831 &
             0.2829 & 0.2842 &
             0.2844 & 0.2844 & 
             0.2831 & 0.2849 \\

            $[0.97, 1.1]$ & 
             0.2859 & 0.2880 & 
             \tbest{0.2796} & 0.2829 &
             0.2829 & \best{0.2847} &
             0.2847 & 0.2847 & 
             0.2833 & \sbest{0.2851} \\

             $[0.98, 1.1]$ & 
             \sbest{0.2863} & 0.2881 & 
             \sbest{0.2798} & \sbest{0.2833} &
             0.2834 & 0.2842 &
             0.2851 & 0.2848 & 
             \best{0.2837} & \sbest{0.2851} \\

             $[0.99, 1.1]$ & 
             0.2860 & \tbest{0.2882} & 
             0.2795 & \tbest{0.2832} &
             \best{0.2836} & 0.2841 &
             0.2851 & \sbest{0.2850} & 
             \tbest{0.2835} & \sbest{0.2851} \\

             $[1.0, 1.1]$ & 
             \best{0.2864} & 0.2881 & 
             0.2795 & 0.2828 &
             \tbest{0.2834} & 0.2842 &
             0.2852 & \best{0.2851} & 
             \sbest{0.2836} & \sbest{0.2851} \\

             $[1.01, 1.1]$ & 
             \tbest{0.2862} & 0.2881 & 
             0.2793 & 0.2828 &
             \tbest{0.2834} & \sbest{0.2844} &
             \best{0.2855} & \tbest{0.2849} & 
             \sbest{0.2836} & \sbest{0.2851} \\

             $[1.02, 1.1]$ & 
             0.2860 & \sbest{0.2883} & 
             \tbest{0.2796} & 0.2828 &
             \best{0.2836} & 0.2840 &
             \sbest{0.2854} & \tbest{0.2849} & 
             \best{0.2837} & \tbest{0.2850} \\

             $[1.03, 1.1]$ & 
             0.2859 & 0.2880 & 
             0.2795 & 0.2824 &
             \sbest{0.2835} & \tbest{0.2843} &
             \sbest{0.2854} & 0.2850 & 
             \sbest{0.2836} & 0.2849 \\

             $[1.04, 1.1]$ & 
             0.2858 & \best{0.2901} & 
             0.2789 & \best{0.2853} &
             0.2830 & 0.2840 &
             \tbest{0.2853} & 0.2847 & 
             0.2833 & \best{0.2860} \\
    

            $[1.05, 1.1]$ & 
             0.2858 & 0.2880 & 
             0.2788 & 0.2820 &
             0.2831 & 0.2839 &
             0.2852 & 0.2842 & 
             0.2832 & 0.2845 \\
          
        
            \hline
        \end{tabular}
        
    }
    \label{tab-sd_turbo_fix_r}
\end{minipage}

==> algorithm-figure-table/tab/tab-sdxl_turbo_best_ablation.tex <==
% SDXL-Turbo 加权 [0.95, 1.15], 重要性得分逆序 (单栏) TODO
\begin{minipage}{1.035\columnwidth}
    \centering
    \captionof{table}{
        SDXL-Turbo Ablation. 
    }
    \hspace{-3em}
    \resizebox{0.98\columnwidth}{!}{
        \centering
        \begin{tabular}{c | c c c c c c c c | c c}
            \hline
            \multirow{2}{*}{\textbf{Weighting}} &
            \multicolumn{2}{c}{\textbf{anime}} & 
            \multicolumn{2}{c}{\textbf{concept-art}} & 
            \multicolumn{2}{c}{\textbf{paintings}} & 
            \multicolumn{2}{c|}{\textbf{photo}} &
            \multicolumn{2}{c}{\textbf{avg}} \\
    
            ~ & 
            train & test & train & test &
            train & test & train & test & 
            train & test \\
    
            \hline

            Vanilla & 
            0.2848 & 0.2898 &
            0.2785 & 0.2815 &
            0.2785 & 0.2812 &
            0.2804 & 0.2818 & 
            0.2801 & 0.2836 \\

            \hdashline

            % \hdashline

            $[0.95, 1.15]^{\text{rev}}$ & 
            \sbest{0.2861} & \sbest{0.2904} & 
            \sbest{0.2791} & \sbest{0.2831} &
            \sbest{0.2802} & \sbest{0.2830} &
            \sbest{0.2820} & \sbest{0.2837} & 
            \sbest{0.2818} & \sbest{0.2851} \\

            $[0.95, 1.15]$ & 
            \best{0.2881} & \best{0.2923} & 
            \best{0.2814} & \best{0.2844} &
            \best{0.2818} & \best{0.2844} &
            \best{0.2833} & \best{0.2848} & 
            \best{0.2837} & \best{0.2865} \\

            \hline
        \end{tabular}
        
    }
    \label{tab-sdxl_turbo_best_ablation}
\end{minipage}


==> algorithm-figure-table/tab/tab-sdxl_turbo_fix_l.tex <==
% SDXL-Turbo 加权 [0.98, ?], [1.02, ?] (单栏)
\begin{minipage}{1.035\columnwidth}
    \centering
    \captionof{table}{
        Enhanced SDXL-Turbo ($l = 0.95$). 
    }
    \hspace{-3em}
    \resizebox{0.98\columnwidth}{!}{
        \centering
        \begin{tabular}{c | c c c c c c c c | c c}
            \hline
            \multirow{2}{*}{\textbf{Weighting}} &
            \multicolumn{2}{c}{\textbf{anime}} & 
            \multicolumn{2}{c}{\textbf{concept-art}} & 
            \multicolumn{2}{c}{\textbf{paintings}} & 
            \multicolumn{2}{c|}{\textbf{photo}} &
            \multicolumn{2}{c}{\textbf{avg}} \\
    
            ~ & 
            train & test & train & test &
            train & test & train & test & 
            train & test \\
    
            \hline

            Vanilla & 
            0.2848 & 0.2898 &
            0.2785 & 0.2815 &
            0.2785 & 0.2812 &
            0.2804 & 0.2818 & 
            0.2801 & 0.2836 \\

            \hdashline

            $[0.95, 1.1]$ & 
             \best{0.2881} & 0.2910 & 
             \best{0.2814} & \sbest{0.2842} &
             \best{0.2819} & \best{0.2847} &
             \best{0.2833} & \sbest{0.2847} & 
             \best{0.2837} & \sbest{0.2862} \\

            $[0.95, 1.15]$ & 
             \best{0.2881} & \best{0.2923} & 
             \best{0.2814} & \best{0.2844} &
             \sbest{0.2818} & \sbest{0.2844} &
             \best{0.2833} & \best{0.2848} & 
             \best{0.2837} & \best{0.2865} \\

             $[0.95, 1.2]$ & 
             \sbest{0.2878} & \sbest{0.2916} & 
             \sbest{0.2810} & 0.2838 &
             0.2816 & 0.2839 &
             \sbest{0.2826} & 0.2842 & 
             \sbest{0.2832} & 0.2859 \\
        
            \hline
        \end{tabular}
        
    }
    \label{tab-sdxl_turbo_fix_l}
\end{minipage}


==> algorithm-figure-table/tab/tab-sdxl_turbo_fix_r.tex <==
% SDXL-Turbo 加权 [?, 1.1] (单栏)
\begin{minipage}{1.035\columnwidth}
    \centering
    \captionof{table}{
        Enhanced SDXL-Turbo ($r = 1.1$). 
    }
    \hspace{-3em}
    \resizebox{0.98\columnwidth}{!}{
        \centering
        \begin{tabular}{c | c c c c c c c c | c c}
            \hline
            \multirow{2}{*}{\textbf{Weighting}} &
            \multicolumn{2}{c}{\textbf{anime}} & 
            \multicolumn{2}{c}{\textbf{concept-art}} & 
            \multicolumn{2}{c}{\textbf{paintings}} & 
            \multicolumn{2}{c|}{\textbf{photo}} &
            \multicolumn{2}{c}{\textbf{avg}} \\
    
            ~ & 
            train & test & train & test &
            train & test & train & test & 
            train & test \\
    
            \hline

            Vanilla & 
            0.2848 & 0.2898 &
            0.2785 & 0.2815 &
            0.2785 & 0.2812 &
            0.2804 & 0.2818 & 
            0.2801 & 0.2836 \\

            \hdashline

            $[0.95, 1.1]$ & 
            \best{0.2881} & 0.2910 & 
            \best{0.2814} & \sbest{0.2842} &
            \best{0.2819} & \best{0.2847} &
            \best{0.2833} & \sbest{0.2847} & 
            \best{0.2837} & \tbest{0.2862} \\

            $[0.96, 1.1]$ & 
            \sbest{0.2880} & \best{0.2925} & 
            \best{0.2814} & 0.2830 &
            \sbest{0.2818} & \sbest{0.2846} &
            \sbest{0.2832} & \best{0.2848} & 
            \sbest{0.2836} & \tbest{0.2862} \\

            $[0.97, 1.1]$ & 
            \sbest{0.2880} & \best{0.2925} & 
            \sbest{0.2813} & \best{0.2843} &
            \tbest{0.2817} & 0.2819 &
            \sbest{0.2832} & \sbest{0.2847} & 
            \sbest{0.2836} & 0.2858 \\

             $[0.98, 1.1]$ & 
             \tbest{0.2879} & \sbest{0.2922} & 
             \tbest{0.2812} & \best{0.2843} &
             0.2816 & \tbest{0.2844} &
             \sbest{0.2832} & 0.2845 & 
             \tbest{0.2835} & \best{0.2864} \\

             $[0.99, 1.1]$ & 
             0.2878 & \tbest{0.2921} & 
             0.2811 & \best{0.2843} &
             0.2814 & 0.2842 &
             \sbest{0.2832} & \best{0.2848} & 
             0.2834 & \sbest{0.2863} \\

             $[1.0, 1.1]$ & 
             0.2877 & 0.2919 & 
             0.2810 & \best{0.2843} &
             0.2814 & 0.2841 &
             \sbest{0.2832} & \tbest{0.2846} & 
             0.2833 & \tbest{0.2862} \\

             $[1.01, 1.1]$ & 
             0.2876 & 0.2917 & 
             0.2811 & \tbest{0.2841} &
             0.2814 & 0.2839 &
             \sbest{0.2832} & 0.2845 & 
             0.2833 & 0.2860 \\

             $[1.02, 1.1]$ & 
             0.2874 & 0.2915 & 
             0.2809 & 0.2839 &
             0.2814 & 0.2838 &
             \sbest{0.2832} & 0.2842 & 
             0.2832 & 0.2859 \\

             $[1.03, 1.1]$ & 
             0.2873 & 0.2915 & 
             0.2807 & 0.2840 &
             0.2813 & 0.2837 &
             \tbest{0.2830} & 0.2841 & 
             0.2830 & 0.2858 \\

             $[1.04, 1.1]$ & 
             0.2873 & 0.2913 & 
             0.2804 & 0.2838 &
             0.2811 & 0.2835 &
             0.2828 & 0.2841 & 
             0.2829 & 0.2857 \\

            $[1.05, 1.1]$ & 
             0.2871 & 0.2913 & 
             0.2802 & 0.2835 &
             0.2811 & 0.2833 &
             0.2828 & 0.2841 & 
             0.2828 & 0.2855 \\
          
        
            \hline
        \end{tabular}
        
    }
    \label{tab-sdxl_turbo_fix_r}
\end{minipage}


==> algorithm-figure-table/tab/tab-skipping_strategy_sdturbo_cat_selected.tex <==
% 表: SD-Turbo, dog 跳过策略 (选)
\begin{table}[t]
    \centering
    \begin{tabular}{c | c c | c}
        \hline
        
        \textbf{Strategy} & \multicolumn{2}{c|}{\textbf{Skipped Block Indices}} & \multirow{2}{*}{\textbf{Note}}  \\
        
        \textbf{Index} & step-0 & step-1 & ~ \\
        
        \hline

        % skip-1: baseline
        a.0 & 0 & 0 & block-0 \\
        a.1 & 1 & 1 & block-1\\
        a.2 & 2 & 2 & block-2 \\
        a.3 & 3 & 3 & block-3 \\
        a.4 & 4 & 4 & block-4\\
        a.5 & 5 & 5 & block-5 \\

        \hdashline

        % skip-1: ours
        b.0 & 1 & 0 & our best \\
        b.2 & 0 & 0 & identical to a.0; our best \\

        \hline

        % skip-2: baseline
        f.0 & 0, 5 & 0, 5 & floor-0 \\
        f.1 & 1, 4 & 1, 4 & floor-1 \\
        f.2 & 2, 3 & 2, 3 & floor-2 \\

        \hdashline

        % skip-2: ours
        g.4 & 1, 4 & 0, 4 & our best \\

        \hline
    \end{tabular}

    \caption{
        Table of skip strategies. 
        We select the static group (a) and the static and symmetric group (f) as baselines. 
        Only the strategies with the best performance in training set or test set from our method are listed. 
        See our supplementary for the full set of strategies. 
    }
    \label{tab-skipping_strategy_sdturbo_dog_selected}
\end{table}

==> algorithm-figure-table/tab/tab-skipping_strategy_sdturbo_fruit_all.tex <==
% SD-Turbo 跳过策略 (全)
\begin{table}[h]
    \centering
    \begin{tabular}{c | c c | c}
        \hline
        
        \textbf{Strategy} & \multicolumn{2}{c|}{\textbf{Skipped Block Indices}} & \multirow{2}{*}{\textbf{Note}}  \\
        
        \textbf{Index} & step-0 & step-1 & ~ \\
        
        \hline

        % skip-1: baseline
        a.0 & 0 & 0 & block-0 \\
        a.1 & 1 & 1 & block-1\\
        a.2 & 2 & 2 & block-2 \\
        a.3 & 3 & 3 & block-3 \\
        a.4 & 4 & 4 & block-4\\
        a.5 & 5 & 5 & block-5 \\
        a.6 & 6 & 6 & block-6 \\

        \hdashline

        % skip-1: ours
        b.0 & 0 & 1 & ~ \\
        b.1 & 0 & 0 & identical to a.0 \\
        b.2 & 1 & 1 & identical to a.1 \\
        b.3 & 1 & 0 & ~ \\

        \hline

        % skip-2: baseline
        c.0 & 0, 6 & 0, 6 & floor-0 \\
        c.1 & 1, 5 & 1, 5 & floor-1 \\
        c.2 & 2, 4 & 2, 4 & floor-2 \\

        \hdashline

        % skip-2: ours
        d.0 & 0, 1 & 0, 1 & ~ \\
        d.1 & 0, 1 & 1, 5 & ~ \\
        d.2 & 0, 1 & 0, 5 & ~ \\
        d.3 & 0, 2 & 0, 1 & ~ \\
        d.4 & 0, 2 & 1, 5 & ~ \\
        d.5 & 0, 2 & 0, 5 & ~ \\
        d.6 & 1, 2 & 0, 1 & ~ \\
        d.7 & 1, 2 & 1, 5 & ~ \\
        d.8 & 1, 2 & 0, 5 & ~ \\

        \hline
    \end{tabular}
    \caption{
        Table of task-specific skipping strategies. 
    }
    \label{tab-skipping_strategy_sdturbo_fruit_all}
\end{table}

==> algorithm-figure-table/tab/tab-voting_score_sd_sdxl_fruit_appx.tex <==
\begin{table}[h]
    \centering
    \caption{
        Dynamic voting score of 20-step SD v2.1/SDXL U-Net, arranged in non-descending order. 
    }
    \begin{tabular}{c | c : c}
        \hline
        \multirow{2}{*}{\textbf{Step}} & 
        \multicolumn{2}{c}{\textbf{Voting Score}} \\

        ~ & SD v2.1 & SDXL \\
        \hline

        0 & 62 65 53 59 63 69 49 & 52 46 47 41 39 \\ 
        1 & 43 76 54 66 59 65 57 & 48 47 41 41 48 \\  
        2 & 57 53 63 82 70 49 46 & 40 45 47 50 43 \\  
        3 & 47 57 53 67 78 62 56 & 46 58 45 45 31 \\  
        4 & 44 58 76 63 70 55 54 & 45 51 52 36 41 \\  
        5 & 32 49 56 66 81 72 64 & 39 52 45 53 36 \\  
        6 & 32 64 72 63 62 61 66 & 40 56 49 48 32 \\  
        7 & 35 64 81 81 64 47 48 & 35 46 60 43 41 \\  
        8 & 40 57 60 86 69 54 54 & 41 54 53 42 35 \\  
        9 & 36 48 59 79 78 62 58 & 38 59 51 50 27 \\  
        10 & 41 56 61 79 72 57 54 & 37 62 53 47 26 \\  
        11 & 39 51 77 68 64 59 62 & 34 55 55 55 26 \\  
        12 & 39 63 78 86 53 42 59 & 35 54 53 59 24 \\  
        13 & 46 59 77 83 59 40 56 & 36 59 54 50 26 \\  
        14 & 39 67 75 90 56 43 50 & 41 49 57 57 21 \\  
        15 & 40 60 80 84 70 51 35 & 39 58 57 49 22 \\  
        16 & 31 64 67 84 76 40 58 & 43 66 53 45 18 \\  
        17 & 48 66 60 85 69 49 43 & 36 60 62 46 21 \\  
        18 & 42 64 79 73 74 42 46 & 33 57 58 55 22 \\  
        19 & 48 66 72 80 86 34 34 & 37 56 57 54 21 \\  
        
        \hline
    \end{tabular}
    \label{tab-voting_score_sd_sdxl_fruit_appx}
\end{table}

==> algorithm-figure-table/tab/tab-voting_score_sdturbo_sdxlturbo_fruit_appx.tex <==
\begin{table}[h]
    \centering
    \caption{
        Dynamic voting score of 2-step SD-Turbo/SDXL-Turbo U-Net, arranged in non-descending order. 
    }
    \begin{tabular}{c | c : c}
        \hline
        \multirow{2}{*}{\textbf{Step}} & 
        \multicolumn{2}{c}{\textbf{Voting Score}} \\

        ~ & SD-Turbo & SDXL-Turbo \\
        \hline

        0 & 26 37 58 87 62 78 72 & 26 39 53 59 48 \\ 
        1 & 40 39 66 84 65 53 73 & 28 40 70 45 42 \\ 

        \hline
    \end{tabular}
    \label{tab-voting_score_sdturbo_sdxlturbo_fruit_appx}
\end{table}
